Towards Practical Oblivious RAM

We take an important step forward in making Oblivious RAM (O-RAM) practical. We propose an O-RAM construction achieving an amortized overhead of 20X-35X (for an O-RAM roughly 1 terabyte in size), about 63 times faster than the best existing scheme. On the theoretic front, we propose a fundamentally novel technique for constructing Oblivious RAMs: specifically, we partition a bigger O-RAM into smaller O-RAMs, and employ a background eviction technique to obliviously evict blocks from the client-side cache into a randomly assigned server-side partition. This novel technique is the key to achieving the gains in practical performance.

==> Makefile <==
# Switched this back to bibtex because the current version of crosstex
# seems to have a bug causing incorrect capitalization in the titles.

LATEX=pdflatex
TEXFLAGS=

TARGET=oram.pdf

all: $(TARGET)

$(TARGET): $(TARGET:.pdf=.tex) *.tex *.bib *.cls Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<

test: test-fonts test-info

test-fonts: $(TARGET)
	pdffonts $<

test-info: $(TARGET)
	pdfinfo $<

print: $(TARGET)
	pdftops $< - | lpr -P lws510

view: $(TARGET)
	kpdf $<

clean:
	rm -f $(TARGET) *.log *.aux *.bbl *.blg *.bak .*.xtx.cache parsetab.py \#*\# *~


==> constant.tex <==

\section{Theoretic Bounds}
\label{sec:proof}
\subsection{Bounding the Partition Size}
\label{sec:boundpartition}
%
%
We now bound the size of each partition.
We will think of the $i$-th cache slot of the client
as an extension of the $i$-th partition on the server. 
We will bound the 
size of the partition plus the corresponding cache slot. 
This is obviously
an upper-bound on the size of the corresponding partition.

We assume that the data access sequence is independent 
of the random coins used in the O-RAM scheme. 
Notice that this is also the case in practical applications.

Suppose we are given a data access sequence:
$$\vec{x} \defeq (x_1, x_2, \ldots, x_M).$$
If we think of the partition and its corresponding
cache slot as a unity, the operations of the O-RAM is equivalent
to the following random process:
Initially, each of the $N$ blocks is assigned to an 
independent random partion.
In each time step, pick an arbitrary element from its corresponding
partition, and place it in a fresh random partition.

Henceforth, when we perform probabilitic analysis on this random process,
we assume that the probability space is defined over the initial coin flips
that place each block into a partition, as well as the coin flips in
each time step $t$ that place $x_t$ into a random partition. 
 


\begin{fact}
At any point of time, the distribution 
of blocks in the partitions (and their extended cache slots)
are the same as throwing $N$ balls into $P$ bins.
\end{fact}
%
%
%

\begin{lemma}
Suppose we throw $N/e$ balls into $N$ bins.
Then, the probability that any bin exceeds
$\frac{(c+1)\log N}{\log\log N} $ balls is bounded by $\frac{1}{N^c}$.
\label{lem:ballbin}
\end{lemma}

\begin{theorem}[Max partition size]
Let $k > 0$, and $M \leq N^k$.
Suppose the number of partitions is $N$.
Given any sequence $\vec{x}$ of length $M$,
let $Z_{i, t}$ denote the size of the partition
$i$ at time step $t$. 
Then,
\[
\Pr\left[\exists i \in [N], t\in [M] : Z_{i,t} > 
\frac{4k \log N}{\log \log N}
\right]
\leq \frac{1}{N} 
\]
\end{theorem}

\begin{proof}
By union bound over the number of data accesses.
\end{proof}



\subsection{Bounding Client Data Cache Size}
We now bound the size of the client's data cache.
Towards this end, we consider the following variant
of the background eviction algorithm.

Recall that in the basic construction, given a data request for
block $\id$, let $p$ denote the current partition or slot associated
with block $\id$.
The alogorithm will perform the following:
1) Fetch block $\id$ (or a dummy block) from
partition $i$, and place block $\id$ into a random slot;
and 2) write back a block to partition $p$ if slot $i$
is filled, and otherwise, write back a dummy block.

\noindent\textbf{Instantiation 
of the background eviction algorithm.}
For the purpose of the proof, we will consider a specific instantiation 
of the background eviction algorithm.
Let $P$ denote the number of partitions.
Given a data request, after performing above normal steps, also
perform the following background eviction algorithm:
for every slot, with probability $\frac{10}{P}$:
evict a real block if the slot is filled, else write back a dummy
block.
%


In the following analysis, we assume that with a data request,
we do not perform the normal eviction, but only the background eviction.
This obviously gives an upper bound on the client cache size. 


Now focus on a single slot. 
A slot can be viewed as a discrete-time Markov Chain
as shown below. Basically,
in every time step, with probability
$p = \frac{1}{P}$, 
a block is added to the slot, and with probability
$q = \frac{10}{P}$, a block is evicted (if one exists).
The Markov Chain is depicted below, where each state
represents the number of blocks in the slot.

%
%
%
\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{mc}
\end{figure}


Let $\rho = \frac{p(1-q)}{q(1-p)} \leq \frac{1}{8}$.
Let $\pi_i$ denote the probability that a slot has 
$i$ blocks in the stationary distribution. Due to standard
Markov Chain analysis, we get: 
\[
\pi_i = \rho^i (1-\rho) 
\]  



\elaine{Choose number of partitions $P = N$.}

\begin{fact}
Let $Z_i$ denote the load of the $i$-th slot at any given
point of time.
\[
E[Z_i] = \frac{\rho}{1-\rho} = \frac{1}{5}
\]
\end{fact}

\begin{fact}
Let $Z$ denote the total number of blocks
in all slots at any given point of time
after the chain has reached stationary distribution.
\[
E[Z] = \frac{1}{5} P \leq \frac{N}{5} 
\]
\end{fact}

\begin{theorem}
After the chain reaches stationary distribution,
\[
\Pr[Z > \frac{N}{5} + c\sqrt{N} ] \leq \frac{1}{N^c}
\]
\end{theorem}
\begin{proof}
It is not hard to show that the 
loads of all slots are negatively associated, using
similar techniques described in \cite{nega}.

Due to \cite{nega}, we can then apply Chernoff bound
\[
\Pr[Z > \frac{N}{5} + k\sqrt{N} ] \leq \frac{1}{N^k}
\]
\end{proof}


\begin{theorem}
Let $M \leq N^k$ for some $k > 0$.
Let $Z(\vec{0}, t)$ denote the total number of blocks in the client
data cache at time $t \in [M]$, 
assuming that the system intitally starts in the state $\vec{0}$, i.e., 
all slots are empty initially.
Then, 
\[
\Pr\left[ \max_{t\in [M]} Z(\vec{0}, t) > 
\frac{N}{5} + (k+1)\sqrt{N} \right] \leq 
\frac{1}{N}
\]
\label{thm:clientcache}
\end{theorem}
\begin{proof}(\textit{sketch.})
Assume that the mixing time 
of the Markov Chain for each slot is $T$.

We show that with high probability, the data cache  
size never exceeds $\frac{N}{5} + (k+1) \sqrt{N}$
between time $T$ and $T + M$.
To show this, simply use Lemma~\ref{lem:cachesingletime}, and take 
take union bound over time steps $T$ through $T+M$:
\[
\Pr\left[ \max_{t\in [T, T+M]} Z(\vec{0}, t)  > \frac{N}{5} + (k + 1)\sqrt{N}  \right] \leq 
\frac{1}{N}
\]
Furthermore, notice that the cache size 
is less likely to exceed a certain upper-bound when each slot starts
empty, than starting in any other initial state. 
Stated formally, 
\begin{align*}
&\Pr\left[ \max_{t\in [M]} Z(\vec{0}, t)  > \frac{N}{5} + (k + 1)\sqrt{N}\right] \\
\leq &
\Pr\left[ \max_{t\in [T, T+M]} Z(\vec{0}, t)  > \frac{N}{5} + (k+1)\sqrt{N} \right] \\
 \leq & \frac{1}{N}
\end{align*}
\end{proof}

\begin{table*}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Scheme} & \multirow{2}{*}{Amortized Cost} & \multirow{2}{*}{Worst-case Cost} & \multirow{2}{*}{Client Storage} & \multirow{2}{*}{Server Storage} & Practical \\ 
& & & & & Performance \\ \hline
\hline
Pinkas-Reinman~\cite{PinkasORAM} & $O((\log N)^2)$ & $O(N \log N)$ & $O(1)$ & $O(N)$ & {\small $60,000 \sim 80,000$X} \\ \hline
{\small Goodrich-Mitzenmacher~\cite{MMORAM}} & $O(\log N)$ & $O(N)$ & $O(\sqrt{N})$ & $O(N)$ &  {\small > $60,000 \sim 80,000$X} \\ \hline
Combined~\cite{PinkasORAM,MMORAM} & $O(\log N)$ & $O(N)$ & $O(\sqrt{N})$ & $O(N)$ & 
$150\sim 250$X \\ \hline
\hline
Theoretic construction & \multirow{2}{*}{{\small $O(\log N (\log \log N)^2)$}} & \multirow{2}{*}{{\small $O((\log N)^2 \log \log N)$}} & \multirow{2}{*}{$O(1)$} & \multirow{2}{*}{$O(N)$} & \multirow{2}{*}{---}\\ 
(This paper) & & & & & \\ \hline
Theoretic variant& \multirow{2}{*}{{\small $O(\log N \log \log N)$}} & \multirow{2}{*}{{\small $O((\log N)^2)$}} & \multirow{2}{*}{$O(\log N)$} & \multirow{2}{*}{$O(N)$} & \multirow{2}{*}{---}\\ 
(This paper) & & & & & \\ \hline
Practical construction & \multirow{2}{*}{$O(\log N)$} & \multirow{2}{*}{$\widetilde{O}(\sqrt{N})$} & \multirow{1}{*}{$c N$} & \multirow{2}{*}{$\widetilde{O}(N)$} & \multirow{2}{*}{20 $\sim$ 35X}\\ 
(This paper) & & & ($c$ very small) &  & \\ \hline
\end{tabular}
\label{tab:contr}
\caption{Our contributions. 
{\normalfont The $\widetilde{O}$ notation hides
to up to a logarithmic factor. For our practical construction, the constant $c$
associated with client-side storage
is very small.
The practical performance is the number of client-server operations per O-RAM operation for typical parameters 
that one would encounter in realistic settings today, e.g., when the
server stores terabytes of data, and the client has several hundred
megabytes to gigabytes of local storage. 
We do not provide practical performance numbers for our theoretic construction,
since we recommend the practical construction to be used in practice.
}}
\end{table*}




==> experiment_figures.tex <==
\section{Experiment Figures}



==> remarks.tex <==
\section{Remarks}

\begin{remark}[Partition O-RAM semantics]
Exisiting O-RAM constructions~\cite{GoldORAM,PinkasORAM,MMORAM}
always perform both a read and a write operation 
upon any data access request.
For the purpose of the partitioning framework,
it helps to separate the reads from the writes. In particular,
we require that a $\pRead$ operation logically removes the fetched block
from the corresponding partition. 
In many existing O-RAM constructions~\cite{PinkasORAM,MMORAM,GoldORAM},
upon a read operation, the block requested is first read, then logically removed
from the O-RAM, and finally added back to the  
first level (a.k.a., cache level).
By ``logically remove'', we mean that the old data block may still
exist in the O-RAM as a stale copy, but will be cleaned out
upon a future reshuffling operation.

Our $\pRead$ operation is the assumed to be the act of reading the specified block and logically removing it from the O-RAM without actually writing back the block to the first level of cache. For some existing O-RAM constructions, two $\pRead$ operations in a row might not be possible, but this can easily be fixed by performing a dummy $\pWrite$ operation in between. As demonstrated later, our constructions perform piggy-backed evictions which ensure that two $\pRead$ operations never happen in a row.

Our $\pWrite$ operation has the same semantics as the write operation of existing O-RAM constructions.

\label{rmk:blackbox}
\end{remark}

